SpinArt: A Spin-based Verifier for Artifact Systems

Data-driven workflows, of which IBM's Business Artifacts are a prime exponent, have been successfully deployed in practice, adopted in industrial standards, and have spawned a rich body of research in academia, focused primarily on static analysis. In previous work, we obtained theoretical results on the verification of a rich model incorporating core elements of IBM's successful Guard-Stage-Milestone (GSM) artifact model. The results showed decidability of verification of temporal properties of a large class of GSM workflows and established its complexity. Following up on these results, the present paper reports on the implementation of SpinArt, a practical verifier based on the classical model-checking tool Spin. The implementation includes nontrivial optimizations and achieves good performance on real-world business process examples. Our results shed light on the capabilities and limitations of off-the-shelf verifiers in the context of data-driven workflows.

==> model.tex <==


\section{Changes Compared to the Previous Model}

\victor{I incorporated these changes in the new definition of the model.}
We consider specification with acyclic schema and no arithmetic. The following restrictions can be removed:
\begin{itemize}\itemsep=0pt\parskip=0pt
\item Arbitrary set of variables (instead of a fixed set) can be used to update the artifact relations
\item There can be multiple artifact relations in each task.
\item When an internal service $\sigma$ is applied, $\sigma$ is allowed to specify any set of variables $\bar{y}$
to propagate to the next instance. The set of variables propagated is $\bar{y} \cup \bar{x}^T_{in}$
\victor{I defined $\bar{y}$ to be the propagated variables, with the constraint that $\bar{x}^T_{in} \subseteq \bar{y} \subseteq \bar{x}^T$}
\item When a child task $T_c$ of $T$ returns, $T_c$ can overwrite any variables of $T$ except $\bar{x}^T_{in}$ (input variables of $T$).
\item Between two internal transitions of the parent task $T$, any child task $T_c$ of $T$ can be called any number of times.
When $T_c$ is called, the previous call to $T_c$ must have returned to $T$.
\end{itemize}

Syntactic sugars added in the new specification language:
\begin{itemize}\itemsep=0pt\parskip=0pt
\item Can insert multiple tuples within one internal transition.
\item Introduce an new type $\mathtt{STR}$ for strings, which can be simulated by the numeric type.
\item Each ID variable is typed with a particular relation
\end{itemize}



\section{Framework}\label{sec:framework}

\victor{No longer needed.}
Database schema $\db$ is a set of relation symbols, where each $R$ has a sequence of attributes
$(\emph{ID}, A_1, \dots, A_n)$ where $\emph{ID}$ is a key attribute and has domain $\dom_R$. 
The domains $\dom_R$ are mutually disjoint for all $R$.
Each attribute $A_i$ has domain either $\mathbb{N}$ or $\dom_{R'}$ for some relation $R' \in \db$. 
The schema also satisfy the inclusion dependencies that for every $R, R' \in db$ where attribute $A$ of $R$ 
has domain $\dom_{R'}$, $R[A] \subseteq R'[\emph{ID}]$.

A database schema $\db$ is acyclic if there are no cycles in the references induced by foreign keys.
% More precisely, consider the labeled graph FK whose nodes are the relations of the schema and in which there is an edge
% from $R_i$ to $R_j$ labeled with $F$ if $R_i$ has a foreign key attribute $F$ referencing $R_j$. The schema $\db$ is {\em acyclic} if the graph FK
% is acyclic

A task schema $T$ is a tuple $(\bar{x}^T, \cals^T)$, where $\bar{x}^T$ is a tuple of artifact variables
and $\cals^T$ is a set of relation symbols not in $\db$. For each relation $\cals \in \cals^T$,
we denote by $\mathtt{attr}(\cals)$ the set of attributes of $\cals$.
The domain of each variable $x \in \bar{x}^T$ and each attribute $A \in \mathtt{attr}(\cals)$
is either $\mathbb{N}$ or $\dom_R \cup \{\anull\}$ for some relation $R \in \db$. 
A variable $x$ or an attribute $A$ has type $R$ (denoted as $\type(x) = R$ or $\type(A) = R$) 
if $dom(x)$ ($dom(A)$) equals $\dom_R \cup \{\anull\}$.
An instance $\rho$ of $T$ is a tuple $(\nu, S_1, \dots, S_k)$ 
where $\nu$ is a valuation of $\bar{x}$ and for each $\cals_i \in \cals^T$, $S_i$ is a set of tuples having 
the type of $\cals_i$.


A service $\sigma$ of task $T$ is a tuple $(\pi, \psi, \bar{y}, \delta)$, 
where $\pi, \psi$ are the pre- and post-condtions, 
$\bar{y} \subseteq \bar{x}^T$ is the set of propagated variables, and $\delta$ is a subset of 
$\{+\cals_i(\bar{z}), -\cals_i(\bar{z}) | \cals_i \in \cals^T, 
\bar{z} \subseteq \bar{x}^T, \type(\bar{z}) = \type(\cals_i) \}$ of size at most 1.
Given two instances $(\nu, S_1, \dots, S_k), (\nu', S_1', \dots, S_k')$ 
of task $T$ and a service $\sigma$, $\rho \goto{\sigma} \rho'$ is a valid transition if
\begin{itemize}\itemsep=0pt\parskip=0pt
\item $\nu \models \pi$, $\nu' \models \psi$,
\item $\nu(\bar{y}) = \nu'(\bar{y})$, and
\item if $\delta = \emptyset$ then $S_i' = S_i$ for all $i$.
If $\delta = \{+\cals_i(\bar{z})\}$, then $S_j' = S_j$ for all $j \neq i$ and
$S_i' = S_i \cup \{ \nu(\bar{z}) \}$.
If $\delta = \{-\cals_i(\bar{z})\}$, then $S_j' = S_j$ for all $j \neq i$ and
$S_i' = S_i - \{ \nu'(\bar{z}) \}$.
\end{itemize}
Note that when $\delta \neq \emptyset$, $\bar{y} = \bar{x}^T_{in}$.




%\section{Outline}
%\begin{itemize}
%\item models: the new hierarchical models, HLTL-FO
%\item new verification result: with acyclic schema, verification is {\sc expspace-complete}.
%\item spin-based verifier
%\item karp-miller-based verifier
%\end{itemize}
%
%Decidability for two cases: multiple-insert-single-retrieve and single-retrieve-multiple-insert
%
%
%
%
%
%Techniques for karp-miller: 
%partial isomorphism types, karp-miller search with pruning, repeated reachability with strongly-connected components,
%pruning with sub-states and super-states
%
%Define isomorphism types and the partial ones.
%
%
%
%
%Static checking on $(=, \neq)$-graphs:
%\begin{itemize}
%\item removing never-violating edges: polynomial algorithm
%\item minimal set of values for assignments
%\end{itemize}
%
%Experiment results














%The arithmetic constraints considered here are over domain $\mathbb{R}$, the real
%numbers. While databases could use non-numeric data, we assume for uniformity, and
%without loss of generality, that all structures are over $\mathbb{R}$. 


%We denote by $\calc$ an infinite set of relation symbols,each of which has a fixed interpretation 
%as the set of solutions of a finite set of linear inequalities with integer
%coefficients. By slight abuse, we sometimes use the same notation for a relation 
%symbol in $\calc$ and its fixed interpretation.

% In this section we present the syntax and semantics of Hierarchical Artifact Systems (HAS's). 
% We begin with the underlying database schema. 
% \vspace{-1mm}
% \begin{definition}
% A \textbf{database schema} $\db$ is a finite set of relation symbols, where 
% each relation $R$ of $\db$ has an associated sequence of distinct attributes 
% containing the following: 
% \vspace{-1mm}
% \begin{itemize}\itemsep=0pt\parskip=0pt
% \item a key attribute $\emph{ID}$ (present in all relations), 
% \item a set of foreign key attributes $\{F_1, \dots, F_m\}$, and
% \item a set of non-key attributes $\{A_1, \dots, A_n\}$ disjoint from \\
% $\{\emph{ID}, F_1, \dots, F_m\}$.
% \end{itemize}
% \vspace{-1mm}
% To each foreign key attribute $F_i$ of $R$ is associated a relation $R_{F_i}$ of $\db$
% and the inclusion dependency $R[F_i] \subseteq R_{F_i}[\emph{ID}]$.
% It is said that $F_i$ references $R_{F_i}$.
% \end{definition} \vspace{-1mm}


% The domain $Dom(A)$ of each attribute $A$ depends on its type. The domain of all non-key attributes is
% numeric, specifically $\mathbb{R}$. 
% The domain of each key attribute is a countable infinite domain disjoint from $\mathbb{R}$.
% For distinct relations $R$ and $R'$, $Dom(R.\emph{ID}) \cap Dom(R'.\emph{ID}) = \emptyset$.
% The domain of a foreign key attribute $F$ referencing $R$ is $Dom(R.\emph{ID})$. We denote by
% $\emph{DOM}_{id} = \cup_{R \in \db} Dom(R.\emph{ID})$. 
% Intuitively, in such a database schema, each
% tuple is an object with a \emph{globally} unique id. This id does not appear
% anywhere else in the database except as foreign keys referencing it.
% An {\em instance} of a database schema $\db$ is a mapping $D$ associating to each relation symbol $R$ a finite relation
% $D(R)$ of the same arity of $R$, whose tuples provide, for each attribute, a value from its domain. In addition,
% $D$ satisfies all key and inclusion dependencies associated with the keys and foreign keys of the schema. 
% The active domain $D$, denoted $\texttt{adom}(D)$, consists of all elements of $D$ (id's and reals). 
% % We denote $\emph{adom}_{id}(D) = \emph{adom}(D) \cap \emph{DOM}_{id}$ and $\emph{adom}_{\mathbb{R}}(D) = \emph{adom}(D) \cap \mathbb{R}$.
% %\yuliang{I think $\emph{adom}_{id}(D)$ and $\emph{adom}_{\mathbb{R}}(D)$ are not used.}
% A database schema $\db$ is {\em acyclic} if there are no cycles in the references induced by foreign keys.
% More precisely, consider the labeled graph FK whose nodes are the relations of the schema and in which there is an edge
% from $R_i$ to $R_j$ labeled with $F$ if $R_i$ has a foreign key attribute $F$ referencing $R_j$. The schema $\db$ is {\em acyclic} if the graph FK
% is acyclic, and it is {\em linearly-cyclic} if each relation $R$ is contained in at most one simple cycle.

% The assumption that the ID of each relation is a single attribute is made for simplicity, and multiple-attribute IDs
% can be easily handled. The fact that the domain of all non-key attributes is numeric is also harmless. 
% Indeed, an uninterpreted domain on which only equality can be used can be easily simulated. 
% Note that the keys and foreign keys used on our schemas are special cases of the dependencies used in \cite{tods12}.
% The limitation to keys and foreign keys is one of the factors leading to improved complexity of verification and still
% captures most schemas of practical interest. 

% We next proceed with the definition of tasks and services, described informally in the introduction.
% The definition imposes various restrictions needed for decidability of verification.
% These are discussed and motivated in Section \ref{sec:undecidability}.

% Similarly to the database schema, we consider two infinite, disjoint sets $\varid$ of ID variables and $\varnum$ of
% numeric variables. We associate to each variable $x$ its {\em domain} $Dom(x)$.
% If $x \in \varid$, then $Dom(x) = \{\anull\} \cup \emph{DOM}_{id}$, 
% where $\anull \not\in \emph{DOM}_{id} \cup \mathbb{R}$
% ($\anull$ plays a special role that will become clear shortly).
% If $x \in \varnum$, then $Dom(x) = \mathbb{R}$. An {\em artifact variable} is a variable in $\varid \cup \varnum$.
% If $\bar{x}$ is a sequence of artifact variables, a {\em valuation} of $\bar{x}$ 
% is a mapping $\nu$ associating to each variable in $\bar{x}$ an element of its domain $Dom(x)$. 

% \vspace{-2mm}
% \begin{definition}
% A \textbf{task schema} over database schema $\db$ is a triple $T = \langle \bar{x}^T, S^T, \bar{s}^T \rangle$ where 
% $\bar{x}^T$ is a sequence of distinct artifact variables, $S^T$ is a relation symbol not in $\db$ with associated arity $k$, and 
% $\bar{s}^T$ is a sequence of $k$ distinct id variables in $\bar{x}^T$. 
% \end{definition}
% \vspace{-1mm}

% We denote by $\bar x^T_{id} = \bar x^T \cap \varid$ and $\bar x^T_{\mathbb{R}} = \bar x^T \cap \varnum$.
% We refer to $S^T$ as the {\em artifact relation} or {\em set} of $T$.
% \vspace{-2mm}
% \begin{definition}
% An \textbf{artifact schema} is a tuple $\mathcal{A} = \langle \calh, \db \rangle$ 
% where $\mathcal{DB}$ is a database schema and $\calh$ is a rooted tree of task schemas over $\db$
% with pairwise disjoint sets of artifact variables and distinct artifact relation symbols.
% \end{definition}\vspace{-1mm}


% The rooted tree $\calh$ defines the {\em task hierarchy}. 
% Suppose the set of tasks is $\{T_1, \ldots, T_k\}$. 
% For uniformity, we always take task $T_1$ to be the root of $\calh$. 
% We denote by $\preceq_\calh$ (or simply $\preceq$ when $\calh$ is understood) the 
% partial order on $\{T_1, \dots, T_k\}$ induced by $\calh$ (with $T_1$ the minimum). For a node $T$ of $\calh$, 
% we denote by $\emph{tree(T)}$ the subtree of $\calh$ rooted at $T$, 
% $\emph{child}(T)$ the set of children of $T$ (also called {\em subtasks} of $T$), 
% $\emph{desc}(T)$ the set of descendants of $T$ (excluding $T$). Finally, $\emph{desc}^*(T)$ denotes
% $\emph{desc}(T) \cup \{T\}$.
% We denote by $\cals_\calh$ (or simply $\cals$ when $\calh$ is understood) the relational schema $\{S^{T_i} \mid 1 \leq i \leq k\}$.
% An instance of $\cals$ is a mapping associating to each $S^{T_i} \in \cals$ a finite relation over $\emph{DOM}_{id}$
% of the same arity.
% \vspace{-2mm}
% \begin{definition}
% An \textbf{instance} of an artifact schema $\mathcal{A} = \langle \calh, \db \rangle $ is a tuple 
% $\bar I = \langle \bar \nu, stg, D, \bar S \rangle$ where 
% $D$ is a finite instance of $\mathcal{DB}$, $\bar S$ a finite instance of $\cals$,
% $\bar{\nu}$ a valuation of 
% $\bigcup_{i=1}^k \bar{x}^{T_i}$, 
% and $stg$ (standing for ``stage'') a mapping of $\{T_1, \dots, T_k\}$ to 
% $\{\ainit, \aactive, \aclosed \}$. 
% \end{definition}
% \vspace{-1mm}

% The stage $stg(T_i)$ of a task $T_i$ has the following intuitive meaning in the context of a run of its parent: 
% $\ainit$ indicates that $T_i$ has not yet been called within the run,  
% $\aactive$ says that $T_i$ has been called and has not returned its answer, and $\aclosed$ indicates that $T_i$
% has returned its answer. As we will see, a task $T_i$ can only be called once within a given run of its parent.
% However, it can be called again in subsequent runs.   

% We denote by $\calc$ an infinite set of relation symbols, each of which has a fixed interpretation 
% as the set of real solutions of a finite set of polynomial inequalities with integer
% coefficients. By slight abuse, we sometimes use the same notation for a relation 
% symbol in $\calc$ and its fixed interpretation.
% For a given artifact schema $\mathcal{A} = \langle \calh, \mathcal{DB} 
% \rangle$ and a sequence $\bar x$ of variables, 
% a {\em condition} on $\bar x$ is a quantifier-free FO formula over 
% $\mathcal{DB} \cup \calc \cup \{=\}$ 
% whose variables are included in $\bar{x}$.
% The special constant $\anull$ can be used in equalities with ID variables.
% For each atom $R(x, y_1, \dots, y_m, z_1, \dots, z_n)$ of relation
% $R(\emph{ID}, A_1, \dots, A_m, F_1, \dots, F_n) \in \db$, 
% $\{x, z_1, \dots, z_n\} \subseteq \varid$ and $\{y_1, \dots, y_m\} \subseteq \varnum$.
% Atoms over $\calc$ use only numeric variables.
% If $\alpha$ is a condition on $\bar x$, 
% $D$ is an instance of $\mathcal{DB}$ and $\nu$ a valuation of $\bar x$, 
% we denote by $D \cup \calc \models \alpha(\nu)$ the fact that $D \cup 
% \calc$ satisfies $\alpha$ with valuation $\nu$ with standard semantics. 
% For an atom $R(\bar{y})$ in $\alpha$ where $R \in \db$ and $\bar{y} \subseteq \bar{x}$,
% if $\nu(y) = \anull$ for any $y \in \bar{y}$, then $R(\bar{y})$ is false.
% %\victor{We need to spell out the semantics when $\nu$ has nulls.} \yuliang{Fixed.}
% %When $\alpha(\nu)$ is evaluated, each relational atom $R(x, y_1, \dots, y_m, z_1, \dots, z_n)$ is \emph{true} iff 
% %$(\nu(x), \nu(y_1), \dots, \nu(y_m), \nu(z_1), \dots, \nu(z_n))$ is in $D(R)$. The standard
% %semantics is used for $\calc$ and $\{=\}$.
% %\yuliang{As an extension, we can have $S^T( \bar{c} )$ for a sequence
% %of constants $\bar{c}$ in conditions.}
% %\victor{Let's decide later on this.}

% % and by CQ$^\neg$ the
% %formulas built from literals (positive and negated atoms) using only conjunction and existential quantification.
% %For each $x_i$, $\emph{desc}(x_i)$ denotes the descendants of $x_i$ in $\calh$ (excluding $x_i$)
% %and $\emph{col}(x_i)$ denotes the set of variables colinear with $x_i$, i.e. descendants or ancestors.

% We next define services of tasks. We start with internal services, which update
% the artifact variables and artifact relation of the task. 
% \vspace{-1mm}
% \begin{definition}
% Let $T = \langle \bar{x}^T, S^T, \bar{s}^T \rangle$ 
% be a task of an artifact schema $\mathcal{A}$.
% An \textbf{internal service} $\sigma$ of $T$
% is a tuple $\langle \pi, \psi, \delta \rangle$ where:
% \vspace*{-1.5mm}
% \begin{itemize}\itemsep=0pt\parskip=0pt
% \item $\pi$ and $\psi$, called \emph{pre-condition} and \emph{post-condition}, 
% respectively, are conditions over $\bar{x}^T$
% \item $\delta \subseteq \{+S^T(\bar{s}^T), -S^T(\bar{s}^T)\}$ is a set of {\em set updates};  
% $+S^T(\bar{s}^T)$ and $-S^T(\bar{s}^T)$ are 
% called the \textbf{insertion} and \textbf{retrieval} of $\bar{s}^T$, respectively. 
% \end{itemize}
% \end{definition}
% \vspace{-1mm}

% Intuitively, $+S^T(\bar{s}^T)$ causes an insertion of the {\em current} value of $\bar{s}^T$ into $S^T$,
% while $-S^T(\bar{s}^T)$ causes the removal of some non-deterministically chosen current tuple of $S^T$
% and its assignment as the {\em next} value of $\bar{s}^T$. In particular, if $\delta = \{+S^T(\bar{s}^T), -S^T(\bar{s}^T)\}$,
% the tuple inserted by $+S^T(\bar{s}^T)$ and the one retrieved by $-S^T(\bar{s}^T)$ are generally distinct, 
% but may be the same as a degenerate case (see definition of the semantics below).

% As will become apparent, although pre-and-post conditions are quantifier-free, $\exists$FO conditions can be simulated 
% by adding variables to $\bar{x}^T$. 

% An internal service of a task $T$ specifies transitions that only 
% modify the variables $\bar{x}^T$ of $T$ and the contents of $S^T$. 
% Interactions among tasks are specified using two kinds of special services, 
% called the \emph{opening-services} and \emph{closing-services}.


% \vspace{-2mm}
% \begin{definition}
% Let $T_c$ be a child of a task $T$ in $\cala$. \\
% (i) The \textbf{opening-service} $\sigma_{T_c}^o$ of $T_c$ is a tuple $\langle 
% \pi, f_{in} \rangle$, where $\pi$ is a condition over $\bar{x}^{T}$, and
% $f_{in}$ is a partial 1-1 mapping from $\bar{x}^{T_c}$ to $\bar{x}^{T}$ (called the input variable mapping).  
% We denote $dom(f_{in})$ by $\bar{x}_{in}^{T_c}$, called the \textbf{input variables} of $T_c$,
% and $range(f_{in})$ by  $\bar x^{T}_{{T_c}^\downarrow}$ (the variables of $T$ passed as input to $T_c$). \\
% (ii) The \textbf{closing-service} $\sigma_{T_c}^c$ of $T_c$ is a tuple $\langle 
% \pi, f_{out} \rangle$, 
% where $\pi$ is a condition over $\bar{x}^{T_c}$,
% and $f_{out}$ is a partial 1-1 mapping from $\bar{x}^{T}$ to $\bar{x}^{T_c}$ (called the output variable mapping). 
% %\yuliang{I think $f_{out}$ is also 1-1.}
% We denote $dom(f_{out})$ by $\bar{x}^{T}_{{T_c}^\uparrow}$, referred to as the \textbf{returned variables} from $T_c$.
% It is required that 
% $\bar{x}_{{T_c}^\uparrow}^{T} \cap {\bar x}_{in}^{T} = \emptyset$.
% We denote by $\bar{x}^{T_c}_{ret}$ the \textbf{to-be-returned variables} (or return variables),
% defined as $range(f_{out})$. 
% %if $T_c$ is a non-root task and otherwise $\emptyset$.
% \end{definition}
% \vspace{-2mm}

% Intuitively, the opening-service  $\langle \pi, f_{in} \rangle$ of a task $T_c$ specifies the condition $\pi$ that the parent task $T$ 
% has to satisfy in order to open $T_c$. When $T_c$ is opened, a subset of the variables of $T$
% are sent to $T_c$ according to the mapping $f_{in}$. 
% Similarly, the closing-service $\langle \pi, f_{out} \rangle$ specifies the 
% condition $\pi$ that $T_c$ has to satisfy in order to be closed and return to $T$. When $T_c$ is closed, a
% subset of $\bar{x}^{T_c}$ is sent back to $T$, as specified by $f_{out}$.


% For uniformity of notation, we also equip the root task $T_1$ with a service $\sigma^o_{T_1}$ with pre-condition {\em true} that initiates 
% the computation by providing a valuation to a designated subset $\bar x^{T_1}_{in}$ of $\bar x^{T_1}$ (the input variables of $T_1$),
% and a service $\sigma^c_{T_1}$ whose pre-condition is \emph{false} 
% (so it never occurs in a run). 
% For a task $T$ we denote by $\Sigma_T$ the set of its internal services,
% $\Sigma_T^{oc} = \Sigma_T \cup \{\sigma^o_T, \sigma^c_T\}$, 
% $\Sigma_T^{\emph{obs}} = \Sigma_T^{oc} \cup \{\sigma^o_{T_c}, \sigma^c_{T_c} \mid T_c \in \emph{child}(T)\}$, and
% $\Sigma_T^\delta = \Sigma_T \cup \{\sigma^o_T\} \cup \{\sigma^c_{T_c} \mid T_c \in \emph{child}(T)\}$.
% Intuitively, $\Sigma_T^{\emph{obs}}$ consists of the services observable in runs of task $T$ 
% and $\Sigma_T^\delta$ consists of services whose application can modify the variables $\bar x^T$. 

% \vspace{-2mm}
% \begin{definition}
% A \emph{Hierarchical Artifact System} (HAS) is a triple $\Gamma = \langle \mathcal{A}, \Sigma, \Pi \rangle$, 
% where $\mathcal{A}$ is an artifact schema, $\Sigma$ is a set of services over $\mathcal{A}$ including 
% $\sigma^o_T$ and  $\sigma^c_T$ for each task $T$ of $\mathcal{A}$, 
% and $\Pi$ is a condition over $\bar x^{T_1}_{in}$  (where $T_1$ is the root task).
% \end{definition}
% \vspace*{-1mm}

% We next define the semantics of HAS's. Intuitively, a run of a HAS on a database $D$ consists of 
% an infinite sequence of transitions among HAS instances (also referred to as configurations, or snapshots), 
% starting from an initial artifact tuple satisfying pre-condition $\Pi$. 
% At each snapshot, each active task $T$ can open a subtask $T_c$ if the pre-condition of the opening service of $T_c$ holds, and the values of
% a subset of $\bar{x}^T$ is passed to $T_c$ as its input variables. $T_c$ can be closed if the pre-condition of
% its closing service is satisfied. When $T_c$ is closed, the values of a subset of $\bar{x}^{T_c}$ are sent to $T$ as
% $T$'s returned variables from $T_c$. An internal service of $T$ can only be applied after all active subtasks of $T$ have returned their answer. 

% \vspace{2mm}
% Because of the hierarchical structure, and the locality of task specifications, 
% the actions of concurrently active children of a given task are independent of each other and can be arbitrarily interleaved.
% To capture just the essential information, factoring out the arbitrary interleavings, we first define the notion
% of {\em local run} and {\em tree of local runs}. Intuitively, a local run of a task consists of a sequence 
% of services of the task, together with the transitions they cause on the task's local artifact variables and relation. 
% The tasks's input and output are also specified. A tree of local runs captures the relationship between 
% the local runs of tasks and those of their subtasks, including the passing of inputs and results.
% Then the runs of the full artifact system simply consist of all legal interleavings
% of transitions represented in the tree of local runs, lifted to full HAS instances (we refer to these as {\em global runs}).  
% We begin by defining instances of tasks and local transitions.
% For a mapping $M$, we denote by $M[a \mapsto b]$ the mapping that sends $a$ to $b$ and agrees with $M$ everywhere else.
% \vspace{-2mm}
% \begin{definition}
% Let $T =  \langle \bar{x}^T, S^T, \bar{s}^T \rangle$ be a task in $\Gamma$ and $D$ a database instance over $\mathcal{DB}$.
% An {\em instance} of $T$ is a pair $(\nu, S)$ where $\nu$ is a valuation of $\bar x^T$ and $S$ an instance of $S^T$.
% For instances $I = (\nu, S)$ and $I' = (\nu', S')$ of $T$ and a service $\sigma \in \Sigma^{obs}_T$,
% there is a local transition $I \goto{\sigma} I'$ if the following holds.
% If $\sigma$ is an internal service $(\pi,\psi)$, then:
% \vspace*{-1mm}
% \begin{itemize}\itemsep=0pt\parskip=0pt
% \item $D \cup \calc \models \pi(\nu)$ and $D \cup \calc \models \psi(\nu')$
% \item $\nu'(y) = \nu(y)$ for each $y$ in $\bar{x}^T_{in}$
% \item if $\delta = \{+S^T(\bar{s}^T)\}$, then $S' = S \cup \{\nu(\bar{s}^T)\}$,
% \item if $\delta = \{-S^T(\bar{s}^T)\}$, then
% $\nu'(\bar{s}^T) \in S$ and $S' =  S - \{\nu'(\bar{s}^T)\}$,
% \item if $\delta = \{+S^T(\bar{s}^T), -S^T(\bar{s}^T)\}$, then
% $\nu'(\bar{s}^T) \in S \cup \{\nu(\bar{s}^T)\}$ and $S' = (S \cup \{\nu(\bar{s}^T)\}) - \{\nu'(\bar{s}^T)\}$, 
% \item if $\delta = \emptyset$ then $S' = S$.
% \end{itemize}
% \vspace*{-1mm}

% If $\sigma =  \sigma^o_{T_c} = \langle \pi, f_{in} \rangle$ is the opening-service for a child $T_c$ of $T$
% then $D \cup \calc \models \pi(\nu)$, $\nu' = \nu$ and $S' = S$.
% If $\sigma = \sigma^c_{T_c}$ then $S = S'$, $\nu'|(\bar x^T - \bar x^T_{T_c \uparrow}) =
% \nu|(\bar x^T - \bar x^T_{T_c \uparrow})$ and $\nu'(z) = \nu(z)$ for every $z \in \bar x^T_{T_c \uparrow} \cap \varid$ for which $\nu(z) \neq \anull$.  Finally, if $\sigma = \sigma^c_T$ then $I' = I$.
% \end{definition}

% \vspace*{-2mm}
% We now define local runs.

% \vspace{-2mm}
% \begin{definition}
% Let $T =  \langle \bar{x}^T, S^T, \bar{s}^T \rangle$ be a non-root task in $\Gamma$ and $D$ a database instance over $\mathcal{DB}$.
% A {\em local run} of $T$ over $D$ is a triple 
% $\rho_T = (\nu_{in}, \nu_{out}, \{(I_i,\sigma_i)\}_{0 \leq i < \gamma})$, where:
% \vspace*{-1mm}
% \begin{itemize}\itemsep=0pt\parskip=0pt
% \item $\gamma \in \mathbb{N} \cup \{\omega\}$
% \item for each $i \geq 0$, $I_i$ is an instance of $T$ and $\sigma_i \in \Sigma^{obs}_T$
% \item $\nu_{in}$ is a valuation of $\bar x^T_{in}$ 
% \item $\sigma_0 = \sigma^o_T$ and $S_0 = \emptyset$,
% \item $\nu_0|{\bar x}^T_{in} = \nu_{in}$, 
% $\nu_0(z) = \anull$ for $z \in \varid- \bar{x}^T_{in}$ and  
% $\nu_0(z) = 0$ for $z \in \varnum -  \bar{x}^T_{in}$ 
% \item if for some $i$, $\sigma_i = \sigma^c_T$ then $\gamma \in \mathbb{N}$ and $i = \gamma-1$ 
% (and $\rho_T$ is called a {\em returning} local run)
% \item $\nu_{out} = \nu_{\gamma-1} |\bar{x}^T_{ret}$ if $\rho_T$ is a returning run and $\bot$ otherwise
% \item a \emph{segment} of $\rho_T$ is a subsequence $\{(I_i,\sigma_i)\}_{i \in J}$, where
% $J$ is a maximal interval $[a, b] \subseteq \{i \mid 0 \leq i < \gamma\}$
% such that no $\sigma_j$ is an internal service of $T$ for $j \in [a + 1, b]$. A segment $J$
% is {\em terminal} if $\gamma \in \mathbb{N}$ and
% $b = \gamma - 1$ (and is called returning if $\sigma_{\gamma-1} = \sigma_T^c$ and blocking otherwise). 
% Segments of ${\rho}_T$ must satisfy the following
% properties. For each child $T_c$ of $T$ there is at most one $i \in J$ such that $\sigma_i = \sigma^o_{T_c}$.
% If $J$ is not blocking and such $i$ exists, there is exactly one $j \in J$ for which $\sigma_j = \sigma^c_{T_c}$, and $j > i$.
% If $J$ is blocking, there is {\em at most} one such $j$.
% %\yuliang{fixed the definition of segments for local runs.} \victor{OK}
% \item for every $0 < i < \gamma$, $I_{i-1} \goto{\sigma_i} I_i$. 
% \end{itemize}
% \vspace*{-1mm}
% Local runs of the root task $T_1$ are defined as above, except that $\nu_{in}$ is a valuation of $\bar x^{T_1}_{in}$ such that
% $D \cup \calc \models \Pi$, and $\nu_{out} = \bot$ (the root task never returns).
% \end{definition}
% \vspace*{-1mm}

% For a local run as above, we denote $\gamma(\rho_T) = \gamma$.
% Note that by definition of segment, a task can call each of its children tasks at most once between two consecutive services in $\Sigma_T^{oc}$
% and all of the called children tasks must complete within the segment, unless it is blocking.  
% These restrictions are essential for decidability and are discussed in Section \ref{sec:undecidability}.
% %Given a local run $\rho_T = (\nu_{in}, \nu_{out}, \{(I_i,\sigma_i)\}_{0 \leq i < \gamma})$, we associate to each $i$ and child $T_c$ of $T$ 
% %a {\em stage} $stg_i(T_c) \in \{\ainit,\aactive,\aclosed\}$ as follows. If $\sigma_i \in \Sigma_T$ then $stg_i(T_c) = \ainit$. 
% %Otherwise, let $J$ be the segment to which $i$ belongs. Then $stg_i(T_c) = \ainit$ if $T_c$ has not been called within $J$,
% %$stg_i(T_c) = \aactive$ if $T_c$ has been called within $J$ and has not yet returned, and $stg_i(T_c) = \aclosed$ if $T_c$ has returned within $J$.
% %Thus, in between two internal services of $T$, each $T_c$ starts in stage $\ainit$, then may be called and transitions to $\aactive$, 
% %and finally may return and move to stage $\aclosed$.  



% Observe that local runs take arbitrary inputs and allow for arbitrary return values from its children tasks.
% The valid interactions between the local runs of a tasks and those of its children is captured by the notion of {\em tree of local runs}.   
% \vspace*{-2mm}
% \begin{definition}
% A {\em tree of local runs} is a directed labeled tree $\Tree$ in which each node
% is a local run ${\rho}_T$ for some task $T$, and every edge connects a local run of
% a task $T$ with a local run of a child task $T_c$ and is labeled with a non-negative integer $i$
% (denoted $i({\rho}_{T_c})$). In addition, the following properties are satisfied.
% Let ${\rho}_T = (\nu^T_{in}, \nu^T_{out}, \{(I_i,\sigma_i)\}_{0 \leq i < \gamma})$ be a node of $\Tree$, where $I_i = (\nu_i, S_i)$, $i \geq 0$.  Let
% $i$ be such that $\sigma_i = \sigma^o_{T_c}$ for some child $T_c$ of $T$. There exists a unique edge
% labeled $i$ from ${\rho}_T$ to a node ${\rho}_{T_c} = (\nu_{in}, \nu_{out}, \{(I'_i,\sigma'_i)\}_{0 \leq i < \gamma'})$
% of $\Tree$, and the following hold:
% \vspace*{-1mm}
% \begin{itemize}\itemsep=0pt\parskip=0pt
% \item $\nu_{in} = f_{in} \circ \nu_i$ 
% where\footnote{Composition is left-to-right.} $f_{in}$ is the input variable mapping of $\sigma_{T_c}^o$
% \item ${\rho}_{T_c}$ is a returning run iff there exists $j > i$ such that $\sigma_j = \sigma^c_{T_c}$;
% let $k$ be the minimum such $j$. Then $\nu_k(z) = \nu_{out}(f_{out}(z))$ for every $z \in \bar x^{T}_{{T_c}^\uparrow}$
% for which $\nu_{k-1}(z) = \anull$, where $f_{out}$ is the output mapping of $\sigma_{T_c}^c$.
% \end{itemize}
% Finally, for every node $\rho_T$ of $\Tree$, if ${\rho}_T$ is blocking then there exists a child of
% ${\rho}_T$ that is not returning (so infinite or blocking).
% \end{definition}
% \vspace*{-1mm}

% Note that a tree of local runs may generally be rooted at a local run of any task of $\Gamma$. 
% We say that $\Tree$ is {\em full} if it is rooted at a local run of $T_1$.

% We next turn to global runs. A global run of $\Gamma$ 
% on database instance $D$ over $\mathcal{DB}$
% is an infinite sequence $\rho = \{ (I_i, \sigma_i) \}_{i \geq 0}$,
% where each $I_i$ is an instance $(\nu_i, stg_i, D, S_i)$ of $\cala$ and $\sigma_i \in \Sigma$,
% resulting from a tree of local runs by interleaving its transitions, lifted to full HAS instances
% (see Appendix B.1 of \cite{arxiv} for the formal definition).  
% For a tree of local runs $\Tree$, we denote by $\call(\Tree)$ the set of all global runs 
% induced by the legal interleavings of $\Tree$. 


